TESDA: Transform Enabled Statistical Detection of Attacks in Deep Neural Networks

Deep neural networks (DNNs) are now the de facto choice for computer vision tasks such as image classification. However, their complexity and "black box" nature often renders the systems they're deployed in vulnerable to a range of security threats. Successfully identifying such threats, especially in safety-critical real-world applications is thus of utmost importance, but still very much an open problem. We present TESDA, a low-overhead, flexible, and statistically grounded method for {online detection} of attacks by exploiting the discrepancies they cause in the distributions of intermediate layer features of DNNs. Unlike most prior work, we require neither dedicated hardware to run in real-time, nor the presence of a Trojan trigger to detect discrepancies in behavior. We empirically establish our method's usefulness and practicality across multiple architectures, datasets and diverse attacks, consistently achieving detection coverages of above 95% with operation count overheads as low as 1-2%.

==> Files/approach_details.tex <==
\subsection{Feature Extraction and Dimensionality Reduction}

In Blocks 2-4 of Figure \ref{fig:singlelayer_flow} the output tensor of each convolutional layer under examination is reduced to a set of PCA coefficients $\theta$ that represents layer behavior. This begins with the Discrete Cosine Transform of Block-2 to extract the frequency components of each convolution kernel output.

\subsubsection{DCT Analysis}

Each convolution kernel in each layer under analysis outputs an image after activation. The DCT \cite{DCT} is used to reduce these images to their frequency components in the form of a sequence of sinusoids (cosines) in two dimensions oscillating at different frequencies. The DCT is taken on the output of each kernel. In this work a single frequency component is chosen for further analysis, with the same component chosen across all kernel outputs' frequency components. This yields a vector of the chosen DCT coefficients $D_i$ for the $i$th layer in the network, with one element for each kernel in the layer. While Trojan trigger presence has been seen to typically affect the higher frequency coefficients \cite{CLEANN}, the flow in Figure \ref{fig:singlelayer_flow} also targets adversarial examples that may not have the same behavior. A range of DCT coefficients is thus tested in this work.

\subsubsection{Principal Component Analysis}\label{PCA_subsec}

For a network of $N$ layers, the procedure outlined above yields a set of $N$ vectors of DCT coefficients $\{D_i\}_{i=1}^N$. 
Each $D_i \in \mathbb{R}^{M_i}$ where $M_i$ is the number of kernels in layer $i$. To further reduce this for attack detection we use Principal Component Analysis (PCA) \cite{PCA} for each layer's vector of DCT coefficients. 

The PCA transforms each $D_i$ to a vector space whose basis vectors are orthogonal to one another. The elements of the transformed vector $T_i$ are ordered according to the energy in each principal component (or basis vector of the transform space), providing an optimal decomposition of $D_i$. As a linear transformation, the PCA has low overhead. The transformation matrix for the $i$th layer is obtained from the mean and covariance of the set of $D_i$ produced across the training data set.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{mlsys2022style/Images/Alphas_plot.png}
    \caption{Graph of Detection Performance versus PCA Coefficient Index ($M$ denotes last PCA coefficient index, $M-1$ last but one until $M-4$ the last but fourth)}
    \label{fig:alphas_choice}
\end{figure}

The vector of DCT coefficients is thus transformed into a vector $T_i=(\alpha_0,\alpha_1,...,\alpha_{M_i})^T$ for each layer $i$, $1\leq i\leq N$. For a dense layer the DCT decomposition is not required and the PCA transform is taken from the output vector of the dense layer for each input to the DNN. The PCA for a dense layer is fitted to the set of outputs produced for each input in the training data set.

One or more elements can then be taken from each $T_i$ for the purposes of outlier detection, reducing the high-dimensional tensor output from a convolutional layer to just a vector containing few coefficients.
% In this work we have taken one element from each transform vector $T_i$.
We note that the higher energy coefficients (e.g., $\alpha_1, \alpha_2$) are seen to contain lesser information about the outliers and therefore have worse detection performance than their lower energy counterparts (e.g., $\alpha_{M_i}$) (Figure \ref{fig:alphas_choice}).
% This is shown in Figure \ref{fig:alphas_choice} for backdoor attacks on PreAct-ResNet-18 \cite{PreactResNet}. The last coefficient is denoted by $M$, the last but one as $M-1$, until the last but fourth $M-4$. \aish{These last couple lines (currently commented out) should be in the caption, not main text.}
In our experiments therefore we restrict ourselves to using just the lowest energy coefficient corresponding to each layer, giving us a vector $\theta \in \mathbb{R}^N$ for every sample, where $\forall i \in \{1,2,...N\},\; \theta_i = \alpha_{M_i}.$

%\aish{Convention is to use lower case letters for vectors and upper case ones for matrices. This section and the one before are a little confusing, would consider re-writing some parts. Made some edits myself.}

\subsection{Attack Detection}

To detect an attack we check if the vector $\theta$ obtained for a particular sample is an \emph{outlier} with respect to the distribution of the clean $\theta$ observed in the training data.
This of course would only hold true if an attack appreciably alters the distribution of the $\alpha$ used in construction of the vector $\theta$, which we confirm empirically to indeed be the case (Figure \ref{fig:example_distribs}).
The presence of an outlier is subsequently assumed to be indicative of abnormal behavior, and hence an attack.
%\aish{Include commented details in fig. caption} %Done, check
% of $\theta$ which is  the distribution of a single layer's chosen $\alpha$ coefficient (here the last $\alpha$ coefficient). This can be seen in Figure \ref{fig:example_distribs}, where an adversarial attack on ResNet-18 dramatically shifts the distribution of the last $\alpha$ coefficient of the second residual unit.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{mlsys2022style/Images/hist_attack_three_densities.jpg}
    \caption{Distributions of the last $\alpha$ for the second computation unit 
    %\aish{Which?} %Done above 
    of ResNet-18 for clean as well as adversarial samples. As observed, the adversarial attack dramatically shifts the lower moments of the distribution. \aish{Why are the probabilities greater than 1? This has to be unnormalized in some way.}} %Displayed as a pdf, this used NumPy's histogram function to normalize a histogram as probabilities/distribution. The area under it is unity.
    \label{fig:example_distribs}
    \vspace{-0.5cm} %Potentially remove, see if paper LaTeX adjusts later
\end{figure}

For the purposes of this work we approximate the distribution of clean $\theta$ across the training set as a \textbf{multidimensional Gaussian} $\mathcal{N}(\mu,\Sigma)$, which lets us take advantage of the well-studied statistical tools available for robust Gaussian parameter estimation and model fitting.
In particular, we leverage the minimum covariance determinant (MCD) method \cite{rousseeuw1984least, rousseeuw1985multivariate, covarianceellipse} to compute $\hat{\mu}, \hat{\Sigma}$ which act as our estimates of the true mean (${\mu}$) and covariance (${\Sigma}$), given the set of $\theta$ across the training set.
An advantage to doing so is knowing that in the case of elliptical (i.e., Gaussian) models, the MCD method has been shown to be asymptotically consistent \cite{butler1993asymptotics}.

The elliptic envelope outlier detector fits this robust mean and covariance estimate to the  $N$-dimensional input data (here the set of $\Theta$ across the training dataset), assuming a certain fraction $\varepsilon$ of the dataset are outliers \cite{hubert2018minimum}. This assumption allows tuning the contamination parameter to achieve a desired threshold for the false positive rate. Provided the training data is an accurate representation of test conditions, contamination parameter $\varepsilon = K$ ideally corresponds to an outlier threshold for $K\%$ false positives. For a test input, the vector $\Theta$ is deemed to be an outlier based on the Mahalanobis distance from the fitted ellipse.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{mlsys2022style/Images/ellipse_example.jpg}
    \caption{Example Outlier Detection for ResNet-18}
    \label{fig:example_ellipse}
\end{figure}

An example of this fit is seen in Figure \ref{fig:example_distribs}. An elliptic envelope was fitted to the set of $\Theta$ from ResNet-18 \cite{Resnet} over CIFAR-10 training data. 100 clean test samples (black dots) and 100 adversarial samples (red dots) were passed through the DNN and detector. The detector was set up across the second computation unit (\textit{Inner layer} axis of the image) and the final layer of the DNN.

\subsubsection{Tuning the Contamination Parameter $\varepsilon$ to Match Target False Positive and False Negative Rates}

Let $\hat{\mu} \in \mathbb{R}^k \textrm{ and positive definite } \hat{\Sigma} \in \mathbb{R}^{k \times k}$ be the sample mean and covariance estimates\footnote{We assume that the total number of samples $n$ is sufficiently large and that the number of adversarial samples $m < n$, such that the sample estimates $\hat{\mu}, \hat{\Sigma}$ converge to the true mean and covariance $\mu, \Sigma$ of the non-contaminated sample.}\textsuperscript{,}\footnote{Specifically, the number of samples over which the minimum covariance determinant is computed, $h = [\frac{n+k+1}{2}]$, where $k$ is the number of features. For our purposes, we can assume $h \approx \frac{n}{2}$. The number of adversarial samples $m \ll n-h \lessapprox \frac{n}{2}$.} provided by the MCD method.
For a sample $\theta$ to be classified as an outlier (i.e., an attack) we require that $d \geq \Delta,$ where $d = {(\theta-\hat{\mu})^T\hat{\Sigma}^{-1}(\theta-\hat{\mu})}$ is the squared Mahalanobis distance of $\theta$ and $\Delta$ is a constant computed over and fit to the entire training data.
Moreover, $\Delta$ depends on the contamination parameter $\varepsilon \in (0,0.5)$ and is defined such that the number of outliers present in the training data $m = \varepsilon n$.

Given that $\varepsilon$ is an upper bound on the contamination of the training set, we want to pick $\Delta$ such that $\mathbb{P}[d \geq \Delta] \leq \varepsilon$.
% At the same time, given that our clean $\theta_i$ are approximated as belonging to the multivariate Gaussian distribution $\mathcal{N}(\hat{\mu},\hat{\Sigma}),$ the distribution of $d_i$ for these $\theta_i$ is given by a chi-squared distribution with $k$ degrees of freedom $\chi_k^2$.
At the same time, by the multivariate Chebyshev inequalty \cite{stellato2017multivariate} we have $\mathbb{P}[d \geq t] \leq \frac{k(n^2 - 4 + 2nt^2)}{n^2t^2}$
% where $n$ is the total number of samples in our training set.
Equating the two probabilities, $\Delta = \sqrt{\frac{k(n^2-4)}{\varepsilon n^2 - 2nk}}$ which in turn implies $\Delta = \mathcal{O}(\sqrt{\frac{k}{\varepsilon}})$ as $n \rightarrow \infty$.

The above expression for $\Delta$ naturally leads to principled ways of choosing the contamination parameter $\varepsilon$ to match (i.e., always stay under) a specified false negative ($\tau_N$) or false positive ($\tau_P$) rate.

False negative rate (FNR) is by definition the complement of the true positive rate (TPR), which on the training set must be $\varepsilon$.
Therefore to minimize FNR, we set $\varepsilon = 1 - \tau_N$ and then fix $\Delta \leq{\sqrt{\frac{k(n^2-4)}{\varepsilon n^2 - 2nk}}} = {\sqrt{\frac{k(n^2-4)}{(1-\tau_N)n^2 - 2nk}}}$.

On the other hand, to minimize false positives we simply require that for clean samples $\mathbb{P}[d \geq \Delta] \leq \tau_P$.
We therefore set $\varepsilon = \tau_P$ and fix $\Delta \geq {\sqrt{\frac{k(n^2-4)}{\varepsilon n^2 - 2nk}}} = {\sqrt{\frac{k(n^2-4)}{(\tau_P)n^2 - 2nk}}}.$

\subsubsection{Deriving a Tighter Bound for Outlier Detection}

Leveraging the fact that the distribution of $d^2$ for clean $\theta$ is given by $\chi_k^2$ (i.e., the chi-squared distribution with $k$ degrees of freedom), it is possible to have bounds tighter than those using Chebyshev's inequality, with the caveat that they might no longer expressible as closed form expressions of elementary functions.

In particular, one could write a Chernoff bound \cite{wainwright2015basic} of the form $\mathbb{P}[d^2 \geq t] \leq exp(-\psi^*_x(t))$ where $\psi^*_x(t)$ is defined as $\sup_{\lambda \geq 0}[\lamda t - \psi(\lambda)],$ and $\psi(\lambda)$ is the logarithm of the moment generating function of $d^2$.
% It is assumed $t \geq \mathbb{E}[d^2]$.
Comparing the inequality dictated by the Chernoff bound with $\mathbb{P}[d^2 \geq \Delta^2] \leq \varepsilon$ subsequently implies that $\Delta^2 = t, \textrm{ but now } \log(\varepsilon) = -\psi^*_x(t)$.
Given the $\chi^2_k$ distribution of $d^2$ we have:
$\psi(\lambda) = -\frac{k}{2}\log(1-2\lambda)$
and
$\psi^*_x(t) = \frac{1}{2}(t-k + k\log(k/t)) = log(1/\varepsilon)$.

Solving for $t, \textrm{ we get } \Delta^2 = -kW(\frac{-\varepsilon^{2/k}}{e})$ where $W$ is the Lambert \emph{W} function whose values may be computed numerically should a tighter bound be desired.
The procedure to choose $\varepsilon$ to match a certain $\tau_P$ or $\tau_N$ remains the same as specified previously but with the expression for $\Delta$ and consequently its dependence on $\varepsilon$ needing to be updated.
%%%%%%%%%%%%ALGO FLOW, EASILY REMOVED IF NEED BE%%%%%%%%%%%%
%\input{mlsys2022style/Files/algo}


==> Files/approach_overview.tex <==
\subsection{Detector Components: Single Layer}\label{singlelayer}

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{mlsys2022style/Images/flowchart_initial_singlelayer_old.jpg}
    \caption{Attack Detection Process for a single layer}
    \label{fig:singlelayer_flow}
\end{figure}

An overview of the proposed detector as applied to a single convolutional layer with $M$ kernels is shown in Figure \ref{fig:singlelayer_flow}.
After convolution, bias addition and activation, each kernel produces an $L\times K$ size image, giving a layer output of an $M\times L\times K$ tensor. The size of this tensor can make direct analysis expensive. The first step is to reduce this to low dimensional features. This is done in blocks 2-4 of Figure \ref{fig:singlelayer_flow}, which takes the layer output from Block 1b (after activation).

% \aish{About fig. 2, it helps for them to be standalone, in some sense. Can we add some details about the different blocks to its caption?}

The first step in feature extraction and dimensionality reduction is the use of the Discrete Cosine Transform (DCT) \cite{DCT} to reduce each kernel output to its frequency coefficients in Block 2. This gives a tensor of frequency coefficients of dimension $M\times L\times K$. One or more of the frequency coefficients from each transformed kernel output may be chosen for further analysis.
Here one DCT coefficient was chosen in Block 3 of Figure \ref{fig:singlelayer_flow} from each transformed kernel output, giving an $M\times 1$ length vector of DCT coefficients.

In Block 4, a Principal Components Analysis (PCA) \cite{PCA} transformation is applied \aish{Or just the output of block 3 across all training samples is projected onto the space defined by its principal compnents?} to the set of $M$-length vectors obtained from Block-3 for all samples in the training set, \aish{Maybe name the outputs of the different blocks? Something like $y_1, y_2$ for output of block 1, 2 would be fine.} producing a vector $\alpha \in \mathbb{R}^{M}$ of PC coefficients.
% where each $\alpha_j, j \in \{1,2,...,M\}$ tells us how much of the transformed spanning the PCs of the chosen set of DCT coefficients.
% The PCA is fit to the set of chosen DCT coefficients from the layer outputs across the training data set. This yields a vector $\alpha \in \mathbb{R}^{M}$ spanning the PCs of 

% an $M$-length vector of projections across the $M$-dimensional vector space of the PCA, with coefficients $[\alpha_0,\alpha_1,...,\alpha_M]^T$ ordered according to significance.
One or more of the $\{\alpha_j\}_{j=1}^M$ can be chosen for attack detection in Blocks 4a and 4b.
As is conventional, we assume $\alpha_1 \geq \alpha_2 \geq ... \alpha_M \geq = 0.$
In the case of dense layers a PCA is taken along the layer output vector directly \aish{You mean the DCT step is by-passed?} and one or more of the $\alpha$s from there can be used for attack detection.

Attack detection is done based on the distribution of the chosen $\alpha$ value. If the $\alpha$ from Block-4 is an outlier with respect to the distribution of the corresponding $\alpha$ over training data, it is assumed to indicate an attack. A distribution is fitted to the $\alpha$ values from the set of chosen DCT coefficients on the training data in Block 4a. This distribution is used to set thresholds for outlier detection post-deployment of the DNN and detector, checking $\alpha$ from Block 4 for outliers which are indicative of an attack. Statistical tests leveraging the training distribution for outlier detection are used here, allowing an adjustment of the threshold to ensure a desired false positive rate.
% While Trojan attacks have been seen to typically affect the higher frequency coefficients \cite{CLEANN}, the flow in Figure \ref{fig:singlelayer_flow} also targets adversarial examples that may not. -Maybe use in the detailed section, reason for low DCT coeffs before ablation proves the concept.

\subsection{Network-Level Detector Deployment}\label{network}

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{mlsys2022style/Images/DNN_Layer_Multidim_Flow.jpg}
    \caption{Attack Detection Process for a DNN}
    \label{fig:DNN_flow}
\end{figure}

The framework described in Section \ref{singlelayer} can be easily generalized to provide detection across the entire DNN. Figure \ref{fig:DNN_flow} shows the deployment of this detection methodology at the network level. Each layer's output is reduced to a chosen $\alpha$ coefficient in the dimensionality reduction and feature extraction blocks. Each of these blocks is identical to Blocks 2-4 of Figure \ref{fig:singlelayer_flow}, yielding a PCA coefficient $\alpha$ chosen from the PCA transformation of the layer output DCT as above. For a network of $N$ layers this yields an $N$ length vector of $\alpha$s, $\Theta$ (in Block 1 of Figure \ref{fig:DNN_flow}). A multidimensional distribution can be fitted to the set of $\theta$s across the training data of the DNN to enable attack detection in Block 2a. If the vector $\theta$ produced during network operation is an outlier with respect to that distribution (as in Block 2b), it is considered indicative of an attack. 

In the following section, the components of this detector are presented in detail, followed by experimental evaluation on state of the art attacks in Section \ref{Experimental}. We discuss experimental results in Section \ref{Discussion} and conclude in Section \ref{Conclusion}.

==> Files/priorwork.tex <==
\subsection{Neural Trojan Attacks}
In this section we review the recent work on Neural Trojans and elaborate on the attacks we explore in this work. Neural Trojans can be inserted in the network via \textit{training data poisoning} \cite{chenliubackdoor17, LiuSrivastavaNT17, BadNets,purdue_trojaning_2018}, \textit{alteration of the training algorithm} either in hardware or software \cite{ClementsBackdoor18,li2018hufu} or at the \textit{binary level on a DNN model stored in memory} \cite{rakin2019tbt,LiuTrojanSIN2}. Attacks involving training data poisoning such as BadNet \cite{BadNets} involve training the DNN using compromised data to alter its decision boundary. Attacks involving alteration of the training algorithm \cite{ClementsBackdoor18,li2018hufu} alter computations while training occurs. Attacks on DNN  binary-level code \cite{rakin2019tbt, rakin2020tbfa} induce malicious behavior by \textit{manipulating weight bits of the network} stored in memory in such a way as to induce  misclassification by the DNN on being presented with a trigger image.

%%%%%%%%%%%%%%%%INPUT AWARE AND TBT GO HERE IN BRIEF%%%%%%%%

\subsection{Adversarial Attacks}
Adversarial attacks can be generated via an optimization problem of finding the minimally distorted image that forces misclassification, which can be approximately solved using the L-BFGS algorithm \cite{LBFGS_attack}. A later one-step method to perturb images for an adversarial attack was the Fast Gradient Sign Method (FGSM) \cite{FGSM}, which used a one-step gradient descent to find the point of minimal loss value either to any other class or to a target class in an $\epsilon$-ball around the clean input and thus perturb the image. Carlini and Wagner's later attack counteracted defenses against FGSM and L-BFGS while aiming to solve the problem of finding the minimally distorted input to force misclassification, using margin loss instead of cross-entropy loss (as in L-BFGS) for the optimization \cite{CarliniWagner}. 

In this work we have tested our proposed scheme on the Projected Gradient Descent attack (PGD) attack. The Projected Gradient Descent (PGD) attack \cite{PGD} is an iterative version of the FGSM with random initialization on the clean input. The PGD attack heuristically searches the samples in the $l_{\infty}$ ball around the clean input which have the highest loss value, and which are thus \textit{most likely} to fool the targeted classifier.

\subsection{Neural Trojan Defenses}
%%%%%%%%%%%%%%%%%%%DEFENSES AGAINST THEM%%%%%%%%%%%%%%%%%%%
Defenses against \textit{Neural Trojans} have been a subject of much recent study. Neural Cleanse \cite{NeuralCleanse} relies on gradient descent to reverse engineer the Trojan triggers for detection of a backdoor in the DNN. DeepInspect \cite{DeepInspect} utilizes DNNs trained to detect probable trigger distributions for attack detection. Neural Cleanse and DeepInspect make use of expensive DNNs or optimizations and are not real-time or on-line, requiring the DNN to be taken offline for analysis. STRIP \cite{STRIP} uses perturbation of the inputs to the DNN to detect Trojan triggers and thus attacks in real time but requires repeated perturbation of and prediction from the input image, incurring high overhead. The DNN training process can also be evaluated to locate parameters of the DNN with abnormal behavior as indicative of an attack \cite{TrojCostofClass,baracaldo2018datapoisoning}, but such methods are unsuitable for online detection post-deployment. CLEANN \cite{CLEANN} uses feature comparisons between the image and outputs to detect the presence of a Trojan trigger and hence an attack in real time, but ideally requires hardware co-design and uses high-overhead methods such as sparse recovery.

%%%%%%%%%%%%%%ADV DEFENSES%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Adversarial Attack Defenses}
Defenses against adversarial attacks have begun at the training stage of the network, using PGD examples for training the network \cite{advsurvey}. Methods such as defensive distillation \cite{Carlini2017b} mask the gradient from the adversarial generation process and thereby defend the model. Input preprocessing \cite{Buckman2018} similarly alters input pixel values to obfuscate the gradient the attacker has to find to establish the minimal perturbation to cause misclassification. However, such methods are still vulerable to attacks such as \cite{CarliniWagner}. YOPO (You Only Propagate Once) \cite{YOPO} accelerates the slow process of generating PGD examples for the training set by reusing the gradient of the model's first layer output when generating PGD examples for training. Methods to establish lower bounds on minimal perturbation \cite{hein2017} needed to misclassify or upper bounds on minimal loss \cite{raghunathan2018} provide trainable `certificates' of model robustness. However, all of these methods are before model deployment. Detection of the adversarial attack post-deployment is used to defend the DNN once it is running. DNN models can be used to classify input as adversarial \cite{Grosse2017}, but such methods are expensive. Statistical tests on the input image to see if it falls inside the training data distribution \cite{Grosse2017} can also be used, but are vulnerable to being bypassed \cite{advsurvey}. Other work checks the consistency of input predictions by estimating prediction uncertainty \cite{Feinman2017}. Such methods are, however, unsuitable for detection of Neural Trojans and can lead to high false positive rates for attacks that find highly minimal perturbations.

%%%%%%%%%%%%%%%%%%%%%%CONTRAST: OUR STUFF%%%%%%%%%%%%%%%%%
